Track-Like Event Analysis at the Baikal-GVD Neutrino Telescope

Reconstructed tracks of muons produced in neutrino interactions provide the precise probe for the neutrino direction. Therefore, track-like events are a powerful tool to search for neutrino point sources. Recently, Baikal-GVD has demonstrated the first sample of low-energy neutrino candidate events extracted from the data of the season 2019 in a so-called single-cluster analysis - treating each cluster as an independent detector. In this paper, the extension of the track-like event analysis to a wider data set is discussed and the first high-energy track-like events are demonstrated. The status of multi-cluster track reconstruction and that of the event analysis are also discussed.

==> ChangeLog <==

2023.02.13	v1	first version.   
2023.04.25	v2	fix "skelecton.tex" to use "\onbehalf{..}" for collaboration. 
2023.06.13	v3	fix typo in "PoStemplate_coll.odt".

